Episodic Reinforcement Learning in Finite MDPs: Minimax Lower Bounds Revisited

In this paper, we propose new problem-independent lower bounds on the sample complexity and regret in episodic MDPs, with a particular focus on the non-stationary case in which the transition kernel is allowed to change in each stage of the episode. Our main contribution is a novel lower bound of $\Omega((H^3SA/\epsilon^2)\log(1/\delta))$ on the sample complexity of an $(\varepsilon,\delta)$-PAC algorithm for best policy identification in a non-stationary MDP. This lower bound relies on a construction of "hard MDPs" which is different from the ones previously used in the literature. Using this same class of MDPs, we also provide a rigorous proof of the $\Omega(\sqrt{H^3SAT})$ regret bound for non-stationary MDPs. Finally, we discuss connections to PAC-MDP lower bounds.

==> figures/mdp_stationary_fixed_s.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm,
semithick]
\tikzstyle{every state}=[fill=white,text=black]

\node[state]                (A)                    {$s_1$};
\node[state, fill=white]    (B) [below right of=A] {$s_g$};
\node[state, fill=white]    (C) [below left  of=A] {$s_b$};

\node[state, fill=white,draw=none]    (RG) [right=0.25cm of B] {$r(s_g)=1$};
\node[state, fill=white,draw=none]    (RB) [left=0.25cm of C] {$r(s_b)=0$};

\path  
	(A)  edge[blue]   node{$\textcolor{blue}{\frac{1}{2}+\epsilon} $} (B)
	(A)  edge[bend right,dashed]   node[below]{$\frac{1}{2}$} (B)
	(A)  edge[bend left,dashed]   node[below]{$\frac{1}{2}$} (C)
	(A)  edge[blue]   node[above left]{$\textcolor{blue}{\frac{1}{2}-\epsilon}$} (C)
	(B)  edge [loop below] node{1} (B)  
	(C)  edge [loop below] node{1} (C)    
	;

\end{tikzpicture}

%\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm,
%                    semithick]
%  \tikzstyle{every state}=[fill=red,draw=none,text=white]
%
%  \node[initial,state] (A)                    {$q_a$};
%  \node[state]         (B) [above right of=A] {$q_b$};
%  \node[state]         (D) [below right of=A] {$q_d$};
%  \node[state]         (C) [below right of=B] {$q_c$};
%  \node[state]         (E) [below of=D]       {$q_e$};
%
%  \path (A) edge              node {0,1,L} (B)
%            edge              node {1,1,R} (C)
%        (B) edge [loop above] node {1,1,L} (B)
%            edge              node {0,1,L} (C)
%        (C) edge              node {0,1,L} (D)
%            edge [bend left]  node {1,0,R} (E)
%        (D) edge [loop below] node {1,1,R} (D)
%            edge              node {0,1,R} (A)
%        (E) edge [bend left]  node {1,0,R} (A);
%\end{tikzpicture}

==> source/app_bpi_lb.tex <==
\section{BPI lower bounds in simplified settings}

\subsection{Lower Bound for $S=4$ and Stage-Dependent Transitions}

\begin{theorem}
	Let $(\histpi, \tau, \recpolicy_\tau)$ be an algorithm that is $(\epsilon, \delta)$-PAC for best policy identification in any finite episodic MDP. Assume that for any MDP $\mdp$, the algorithm satisfies $\PPs{\histpi,\mdp}{\tau < \infty} = 1$. Then, there exists an MDP $\mdp$ with stage-dependent transitions such that  for $\epsilon \leq (H/2-1)/8$ and $H \geq 4$,
	\[\EEs{\histpi, \mdp}{\tau} \geq \frac{1}{1024} \frac{H^3 A}{\epsilon^2}\log\pa{\frac{1}{2.4\delta}}\,.\]
\end{theorem}

\begin{proof}
	We consider the same set of MDPs parameterized by $(h^*, a^*) \in \braces{2,\ldots, \overline{H}+1}\times\cA$ as in the proof of Theorem \ref{theorem:regret-non-stationary-fixed-s}, with a slight modification to the function $\Delta_{(h^*, a^*)}(h, a)$ used to define the transition probabilities. Let $(h_0, a_0)  \in \braces{2,\ldots, \overline{H}+1}\times\cA$ be the parameters of a reference MDP. We define
	\begin{align*}
	\Delta_{(h^*, a^*)}(h, a) = \indic{a=a_0, h=h_0}\widetilde{\epsilon} + \indic{a=a^*, h=h^*}2 \widetilde{\epsilon}
	\end{align*}
	where $\widetilde{\epsilon} \eqdef \epsilon/(H-\overline{H}-1)$.
	
	\paragraph{Suboptimality gap of $\recpolicy_\tau$} The value of the optimal policy in any of the MDPs $\mdp_{(h^*, a^*)}$ for $(h^*, a^*)\neq(h_0, a_0)$ is
	\begin{align*}
	\rho^* = (H-\overline{H}-1)\pa{\frac{1}{2} + 2\widetilde{\epsilon}},
	\end{align*}
	and the value of the recommended policy $\recpolicy_\tau$ is
	\begin{align*}
	\rho_{(h^*, a^*)}^{\recpolicy_\tau} = (H-\overline{H}-1)\pa{\frac{1}{2} + 2\,\widetilde{\epsilon}\, \bfPPsu{(h^*, a^*)}{\recpolicy_\tau}{S_{h^*} = s_1, A_{h^*}=a^*}}
	\end{align*}
	where $\bfPP_{(h^*, a^*)}^{\recpolicy_\tau}$ is the probability distribution over the states and actions $(S_h, A_h)_{h\in[H]}$ following the recommended Markov policy $\recpolicy_\tau$ in the MDP $\mdp_{(h^*, a^*)}$. Notice that $\rho_{(h^*, a^*)}^{\recpolicy_\tau}$ is a random variable that is $\cF_H^\tau$-measurable.
	
	\paragraph{Definition of a ``good'' event $E_{(h^*, a^*)}$ in $\mdp_{(h^*, a^*)}$} Since the dynamics of all MDPs are the same up to the moment where $s_1$ is reached, which depends only on $\recpolicy_\tau$, we have
	\begin{align*}
	\bfPPsu{(h_1, a_1)}{\recpolicy_\tau}{S_{h^*} = s_1, A_{h^*}=a^*} = \bfPPsu{(h_2, a_2)}{\recpolicy_\tau}{S_{h^*} = s_1, A_{h^*}=a^*}
	\end{align*}
	for any $(h_1, a_1), (h_2, a_2) \in \braces{2,\ldots, \overline{H}+1}\times\cA$. Hence, we denote
	\begin{align*}
	\bfPPsu{(h^*, a^*)}{\recpolicy_\tau}{S_{h^*} = s_1, A_{h^*}=a^*} = \bfPPu{\recpolicy_\tau}{S_{h^*} = s_1, A_{h^*}=a^*}
	\end{align*}
	\todoOm{explain better this part above}
	
	We define the following event:
	\begin{align*}
	E_{(h^*, a^*)}^\tau \eqdef \braces{ \bfPPu{\recpolicy_\tau}{S_{h^*} = s_1, A_{h^*}=a^*} > \frac{1}{2}  }
	\end{align*}
	
	Since the algorithm is assumed to be $(\epsilon,\delta)$-PAC, we have
	\begin{align*}
	\PPs{(h^*, a^*)}{ E_{(h^*, a^*)}^\tau  } = \PPs{(h^*, a^*)}{\rho^{\recpolicy_\tau} > \rho^* - \epsilon}
	\geq 1-\delta
	\end{align*}
	for all $(h^*, a^*)\neq(h_0, a_0)$. Notice that
	\begin{align*}
	\sum_{(h', a')} \bfPPu{\recpolicy_\tau}{S_{h'} = s_1, A_{h'}=a'} = \sum_{h'} \bfPPu{\recpolicy_\tau}{S_{h'} = s_1} = 1
	\end{align*}
	since, at some point, the state $s_1$ will be reached. This implies that, if there exists $(h_1, a_1)$ such that $\bfPPu{\recpolicy_\tau}{S_{h_1} = s_1, A_{h_1}=a_1} > 1/2$, then, for any other $(h_2, a_2) \neq (h_1, a_1)$ we have $\bfPPu{\recpolicy_\tau}{S_{h_1} = s_1, A_{h_1}=a_1} < 1/2$.
	
	Consequently, for any pair $(h',a')\neq (h^*, a^*)$, we have
	\begin{align*}
	\PPs{(h^*, a^*)}{ E_{(h', a')}^\tau  } & =
	\PPs{(h^*, a^*)}{ \bfPPu{\recpolicy_\tau}{S_{h'} = s_1, A_{h'}=a'} > \frac{1}{2}  } \\
	& \leq \PPs{(h^*, a^*)}{ \bfPPu{\recpolicy_\tau}{S_{h^*} = s_1, A_{h^*}=a^*} < \frac{1}{2}} \\
	& \leq \delta.
	\end{align*}
	
	\paragraph{Lower bound on the expectation of $\tau$ in the reference MDP $\mdp_{(h_0, a_0)}$} Let
	\begin{align*}
	N_{(h^*, a^*)}(\tau) = \sum_{t=1}^\tau \indic{S_{h^*}^t = s_1, A_{h^*}^t = a^*}
	\end{align*}
	such that $\tau = \sum_{(h^*,a^*)} 	N_{(h^*, a^*)}(\tau)$.
	For any $\cF_H^\tau$-measurable random variable $Z$ taking values in $[0, 1]$, we have
	\begin{align*}
	& \EEs{(h_0, a_0)}{N_{(h^*, a^*)}(\tau)} \frac{16\epsilon^2}{(H-\overline{H}-1)^2} \\
	&   \geq \EEs{(h_0, a_0)}{N_{(h^*, a^*)}(\tau)} \kl\pa{\frac{1}{2}, \frac{1}{2}+2\widetilde{\epsilon}} \geq \kl\pa{\EEs{(h_0, a_0)}{Z}, \EEs{(h^*, a^*)}{Z}}.
	\end{align*}
	for any $(h^*, a^*) \neq (h_0, a_0)$ provided that $\widetilde{\epsilon} \leq 1/8$.
	\todoOm{prove the inequality above}
	Letting $Z = \indic{E_{(h^*, a^*)}^\tau}$ yields
	\begin{align*}
	\kl(\EEs{(h_0, a_0)}{Z}, \EEs{(h^*, a^*)}{Z})
	& = \kl\pa{\PPs{(h_0, a_0)}{E_{(h^*, a^*)}^\tau}, \PPs{(h^*, a^*)}{E_{(h^*, a^*)}^\tau}} \\
	& \geq \kl(\delta, 1-\delta) \geq \log\pa{\frac{1}{2.4\delta}}.
	\end{align*}
	\todoOm{citation/proof for inequality above}
	Consequently,
	\begin{align*}
	\EEs{(h_0, a_0)}{N_{(h^*, a^*)}(\tau)} \geq \frac{(H-\overline{H}-1)^2}{16\epsilon^2}\log\pa{\frac{1}{2.4\delta}}
	\end{align*}
	and
	\begin{align*}
	\EEs{(h_0, a_0)}{\tau}
	& \geq \sum_{(h^*,a^*)\neq (h_0, a_0)}\EEs{(h_0, a_0)}{N_{(h^*, a^*)}(\tau)}
	\geq  \frac{(\overline{H}A-1)(H-\overline{H}-1)^2}{16\epsilon^2}\log\pa{\frac{1}{2.4\delta}}\\
	& \geq \frac{1}{2^{10}} \frac{H^3 A}{\epsilon^2}\log\pa{\frac{1}{2.4\delta}}.
	\end{align*}
	by taking $\overline{H} = H/2$ with $H\geq 4$.
	
\end{proof}


==> source/app_regret_lb.tex <==
\section{Regret lower bounds in simplified settings}

\subsection{Lower Bound for $S=3$ and Stage-Independent Transitions}

\begin{theorem}
	For any algorithm $(\histpi, \tau, \recpolicy_\tau)$, there exists an MDP $\mdp_{\histpi}$ whose transitions do not depend on the stage $h$, such that for $T\geq 2A$,
	\[\regret_T(\histpi, \mdp_{\histpi}) \geq \frac{1}{32\sqrt{2}}H\sqrt{AT}\,.\]
\end{theorem}
\begin{proof}
	Consider an MDP with 3 states: an initial state $s_1$, a ``bad'' $s_b$ and a ``good'' state $s_g$. The reward function depends only on the state and is $1$ only in $s_g$, $r_h(s) = \indic{s=s_g}$. The initial state distribution $\mu$ is the Dirac measure at $s_1$ and the transitions are given by:
	\begin{align*}
	& p_h(s_g|s_g, a) = 1 \\
	& p_h(s_b|s_b, a) = 1 \\
	& p_h(s_g|s_1, a) = \frac{1}{2} +  \indic{a=a^*}\epsilon \\
	& p_h(s_b|s_1, a) = \frac{1}{2} -  \indic{a=a^*}\epsilon
	\end{align*}
	that is, both the good and the bad states are absorbing, the transitions from $s_1$ to $(s_g, s_b)$ are uniform and there is one optimal action $a^*$ that increases by $\epsilon$ the probability of getting to the good (rewarding) state. Figure~\ref{fig:mdp-stationary-fixed-s} illustrates this MDP.

	\begin{figure}[ht]
		\centering
		\input{figures/mdp_stationary_fixed_s.tex}
		\caption{MDP used to prove the lower bound for $S=3$ and stage-independent transitions. The filled and dashed lines represent the transitions under action $a^*$ and $a\neq a^*$, respectively.}
		\label{fig:mdp-stationary-fixed-s}
	\end{figure}


	We denote the MDP described above by $\mdp_{a^*}$, and, for a fixed algorithm $(\histpi, \tau, \recpolicy_\tau)$, we define $\P_{a^*} \eqdef\P_{\histpi, \mdp_{a^*}}$ and $\E_{a^*} \eqdef\E_{\histpi, \mdp_{a^*}}$. We also define $\mdp_0$ as the MDP where there is no optimal action, that is, $p_h(s_g|s_1, a) = 1/2$ for all $a\in\cA$.

	\paragraph{Regret of $\histpi$ in $\mdp_{a^*}$} The mean reward gathered by $\histpi$ in $\mdp_{a^*}$ is given by
	\begin{align*}
	\EEs{a^*}{\sum_{t=1}^T\sum_{h=1}^H r_h(S_h^t, A_h^t)}
	= \sum_{t=1}^T \EEs{a^*}{\sum_{h=1}^H \indic{S_h^t = s_g}}
	= (H-1)\sum_{t=1}^T \PPs{a^*}{S_2^t = s_g}.
	\end{align*}
	Since
	\begin{align*}
	\PPs{a^*}{S_2^t = s_g} = \frac{1}{2} + \epsilon \PPs{a^*}{S_1^t = s_1, A_1^t=a^*} = \frac{1}{2} + \epsilon \PPs{a^*}{A_1^t=a^*},
	\end{align*}
	we have
	\begin{align*}
	\rho^* = (H-1)\pa{\frac{1}{2}+\epsilon}
	\quad\text{and}\quad
	\EEs{a^*}{\sum_{t=1}^T\sum_{h=1}^H r_h(S_h^t, A_h^t)} = (H-1)\pa{\frac{1}{2}+\epsilon \EEs{a^*}{\sum_{t=1}^{T}\indic{A_1^t=a^*}}}
	\end{align*}
	and the regret of $\histpi$ in $\mdp_{a^*}$ is
	\begin{align*}
	\regret_T(\histpi, \mdp_{a^*}) =  T(H-1)\epsilon\pa{1-\frac{1}{T}\EEs{a^*}{N_{a^*}}}
	\end{align*}
	where $N_{a^*} \eqdef \sum_{t=1}^{T}\indic{A_1^t=a^*}$ is the number of times the optimal action is chosen in $s_1$.

	\paragraph{Maximum regret of $\histpi$ over all possible $\mdp_{a^*}$} We have
	\begin{align}
	\label{eq:aux1}
	\max_{a^*\in\cA} \regret_T(\histpi, \mdp_{a^*}) \geq \frac{1}{A}\sum_{a^*\in\cA} \regret_T(\histpi, \mdp_{a^*}) = T(H-1)\epsilon\pa{1-\frac{1}{AT}\sum_{a^*\in\cA}\EEs{a^*}{N_{a^*}}}.
	\end{align}

	\paragraph{Upper bound on $\sum_{a^*}\EEs{a^*}{N_{a^*}}$}  Since $N_{a^*}/T \in [0, 1]$, Lemma \ref{lemma:kl-contraction} gives us
	\begin{align*}
	\kl\pa{\frac{1}{T}\EEs{0}{N_{a^*}}, \frac{1}{T}\EEs{a^*}{N_{a^*}}} \leq \KL\pa{\P_{0}^{\hist_H^T}, \P_{a^*}^{\hist_H^T}}.
	\end{align*}
	By Pinsker's inequality, $(p-q)^2 \leq (1/2)\kl(p, q)$, which implies

	\begin{align*}
	\frac{1}{T}\EEs{a^*}{N_{a^*}} \leq \frac{1}{T}\EEs{0}{N_{a^*}} +\sqrt{\frac{1}{2}\KL\pa{\P_{0}^{\hist_H^T}, \P_{a^*}^{\hist_H^T}}}.
	\end{align*}
	Lemma~\ref{lemma:kl-between-mdps} yields
	\begin{align*}
	\KL\pa{\P_{0}^{\hist_H^T}, \P_{a^*}^{\hist_H^T}} = \EEs{0}{N_{a^*}}\kl(1/2, 1/2+\epsilon)
	\end{align*}
	since $\mdp_0$ and $\mdp_{a^*}$ only differ at $(s, a) = (s_1, a^*)$ which can only be visited at $h=1$.

	Assuming that $\epsilon \leq 1/4$, we have $\kl(1/2, 1/2+\epsilon) \leq 4\epsilon^2$ by Lemma \ref{lemma:kl-epsilon}, and, consequently
	\todoOm{prove that $\kl(1/2, 1/2+\epsilon) \leq 4\epsilon^2$} 
	\todoe{Inequality (14.6) in Csaba's book}
	\begin{align*}
	\frac{1}{T}\EEs{a^*}{N_{a^*}} \leq \frac{1}{T}\EEs{0}{N_{a^*}} +  \sqrt{2}\epsilon \sqrt{\EEs{0}{N_{a^*}}}.
	\end{align*}
	Averaging over $a^*\in\cA$ and using the fact that $\sum_{a^*}N_{a^*} = T$, we obtain
	\begin{align}
	\frac{1}{AT}\sum_{a^*}\EEs{a^*}{N_{a^*}} & \leq \frac{1}{A} + \frac{\sqrt{2}\epsilon}{A} \sum_{a^*}\sqrt{\EEs{0}{N_{a^*}}} \nonumber\\
	& \leq \frac{1}{A} + \frac{\sqrt{2}\epsilon}{A}\sqrt{AT}
	\quad\text{by the Cauchy-Schwarz inequality.} \label{eq:aux2}
	\end{align}


	\paragraph{Optimizing $\epsilon$} Putting together equations \eqref{eq:aux1} and \eqref{eq:aux2}, we obtain
	\begin{align*}
	\max_{a^*\in\cA} \regret_T(\histpi, \mdp_{a^*})
	\geq
	T(H-1)\epsilon\pa{1- \frac{1}{A} - \frac{\sqrt{2}\epsilon}{A}\sqrt{AT} }.
	\end{align*}
	Choosing $\epsilon = (2\sqrt{2})^{-1}(1-1/A)\sqrt{A/T}$ and assuming $A\geq 2$ and $H\geq 2$ we obtain
	\begin{align*}
	\max_{a^*\in\cA} \regret_T(\histpi, \mdp_{a^*})
	\geq \frac{1}{4\sqrt{2}}\pa{1-\frac{1}{A}}^2(H-1)\sqrt{AT} \geq \frac{1}{32\sqrt{2}} H\sqrt{AT}.
	\end{align*}
	Finally, notice that the assumption $\epsilon\leq 1/4$ is satisfied if $T\geq 2A$.
\end{proof}

% ==================================================================================

\subsection{Lower Bound for $S=4$ and Stage-Dependent Transitions}


\begin{theorem}
	\label{theorem:regret-non-stationary-fixed-s}
	For any algorithm $(\histpi, \tau, \recpolicy_\tau)$, there exists an MDP $\mdp_{\histpi}$ whose transitions depend on the stage $h$, such that  if $H \geq 4$ and $T\geq HA$,
	 \[\regret_T(\histpi, \mdp_{\histpi}) \geq \frac{1}{128} \sqrt{H^3AT}\,.\]
\end{theorem}
\begin{proof}
	Consider an MDP with 4 states: a ``waiting state'' $s_\mathrm{w}$, an initial state $s_1$, a ``bad'' $s_b$ and a ``good'' state $s_g$. The initial state distribution $\mu$ is the Dirac measure at $s_\mathrm{w}$.
	Let $\overline{H} \in [H]$ be a fixed stage, and $(h^*, a^*) \in \braces{2,\ldots, \overline{H}+1}\times\cA$ be two parameters defining the MDP, such that the reward function and the transitions are
	\begin{align*}
	r_h(s) = \indic{s = s_g, h \geq \overline{H}+2}
	\end{align*}
	and
	\begin{align*}
	& p_h(s_\mathrm{w}|s_\mathrm{w}, a) = \indic{a =  a_\mathrm{w}, h \leq \overline{H}} \\
	& p_h(s_1|s_\mathrm{w}, a) = 1 -  p_h(s_\mathrm{w}|s_\mathrm{w}, a)  \\
	& p_h(s_g|s_1, a) = \frac{1}{2} +  \Delta_{(h^*, a^*)}(h, a)  \\
	& p_h(s_b|s_1, a) = \frac{1}{2} -  \Delta_{(h^*, a^*)}(h, a) \\
	& p_h(s_b|s_b, a) = 1 \\
	& p_h(s_g|s_g, a) = 1
	\end{align*}
	where $\Delta_{(h^*, a^*)}(h, a) = \indic{a=a^*, h=h^*}\epsilon$. That is, the agent starts at $s_\mathrm{w}$ and can choose either to stay in this state by taking the action $a_\mathrm{w}$ or go to $s_1$ by taking any other action. After the stage $\overline{H}$, the agent can no longer stay at $s_\mathrm{w}$ and goes to $s_1$ with probability $1$. There is only a stage $h^*$ where the agent can take a ``good'' action $a^*$ that increases the probability of getting to the rewarding state $s_g$. Intuitively, in addition to identifying the good action $a^*$, the agent also has to learn the good moment $h^*$ to take it, which will result in an extra $\sqrt{H}$ factor in the lower bound.  Figure \ref{fig:mdp-non-stationary-fixed-s} illustrates this MDP.

	\begin{figure}[ht]
		\centering
		\input{figures/mdp_non_stationary_fixed_s.tex}
		\caption{MDP used to prove the lower bound for $S=4$ and non-stationary transitions.}
		\label{fig:mdp-non-stationary-fixed-s}
	\end{figure}

	We denote the MDP described above by $\mdp_{(h^*, a^*)}$, and, for a fixed algorithm $(\histpi, \tau, \recpolicy_\tau)$, we define $\P_{(h^*, a^*)} \eqdef\P_{\histpi, \mdp_{(h^*, a^*)}}$ and $\E_{(h^*, a^*)} \eqdef\E_{\histpi, \mdp_{(h^*, a^*)}}$. We also define $\mdp_0$ as the MDP where there is no optimal action, that is, $p_h(s_g|s_1, a) = 1/2$ for all $(h, a)$.

	\paragraph{Regret of $\histpi$ in $\mdp_{(h^*, a^*)}$} The mean reward gathered by $\histpi$ in $\mdp_{(h^*, a^*)}$ is given by
	\begin{align*}
	\EEs{(h^*, a^*)}{\sum_{t=1}^T\sum_{h=1}^H r_h(S_h^t, A_h^t)}
	& = \sum_{t=1}^T \EEs{(h^*, a^*)}{\sum_{h=\overline{H}+2}^H \indic{S_h^t = s_g}} \\
	& = (H-\overline{H}-1)\sum_{t=1}^T \PPs{(h^*, a^*)}{S_{\overline{H}+2}^t = s_g}.
	\end{align*}
	Since, for any $h \in \braces{2, \ldots, \overline{H}+1}$,
	\begin{align*}
	\PPs{(h^*, a^*)}{S_{h+1}^t = s_g} =
	\PPs{(h^*, a^*)}{S_{h}^t = s_g} + \frac{1}{2}\PPs{(h^*, a^*)}{S_{h}^t = s_1} + \indic{h=h^*}\PPs{(h^*, a^*)}{S_{h}^t = s_1, A_{h}^t=a^*}\epsilon.
	\end{align*}
	Using the facts that $\PPs{(h^*, a^*)}{S_{2}^t = s_g} = 0$ and $\sum_{h=2}^{\overline{H}+1}\PPs{(h^*, a^*)}{S_{h}^t = s_1} = 1$, we obtain
	\begin{align*}
	\PPs{(h^*, a^*)}{S_{\overline{H}+2}^t = s_g} = \frac{1}{2} + \epsilon \PPs{(h^*, a^*)}{S_{h^*}^t = s_1, A_{h^*}^t=a^*}.
	\end{align*}
	Hence, the regret of $\histpi$ in $\mdp_{(h^*, a^*)}$ is
	\begin{align*}
	\regret_T(\histpi, \mdp_{(h^*, a^*)}) =  T(H-\overline{H}-1)\epsilon\pa{1-\frac{1}{T}\EEs{(h^*, a^*)}{N_{(h^*, a^*)}}}
	\end{align*}
	where $N_{(h^*, a^*)} \eqdef \sum_{t=1}^T \indic{S_{h^*}^t = s_1, A_{h^*}^t=a^*}$.


	\paragraph{Maximum regret of $\histpi$ over all possible $\mdp_{(h^*,a^*)}$} We have
	\begin{align}
	\label{eq:aux3}
	\max_{(h^*,a^*)} \regret_T(\histpi, \mdp_{(h^*,a^*)}) & \geq \frac{1}{\overline{H}A}\sum_{(h^*,a^*)} \regret_T(\histpi, \mdp_{(h^*,a^*)}) \nonumber
	\\
	& = T(H-\overline{H}-1)\epsilon\pa{1-\frac{1}{\overline{H}AT}\sum_{(h^*,a^*)}\EEs{(h^*,a^*)}{N_{(h^*,a^*)}}}.
	\end{align}

	\paragraph{Upper bound on $\sum_{(h^*,a^*)}\EEs{(h^*,a^*)}{N_{(h^*,a^*)}}$}  Since $N_{(h^*,a^*)}/T \in [0, 1]$, Lemma \ref{lemma:kl-contraction} gives us
	\begin{align*}
	\kl\pa{\frac{1}{T}\EEs{0}{N_{(h^*,a^*)}}, \frac{1}{T}\EEs{(h^*,a^*)}{N_{(h^*,a^*)}}} \leq \KL\pa{\P_{0}^{\hist_H^T}, \P_{(h^*,a^*)}^{\hist_H^T}}.
	\end{align*}
	By Pinsker's inequality, $(p-q)^2 \leq (1/2)\kl(p, q)$, which implies

	\begin{align*}
	\frac{1}{T}\EEs{(h^*,a^*)}{N_{(h^*,a^*)}} \leq \frac{1}{T}\EEs{0}{N_{(h^*,a^*)}} +\sqrt{\frac{1}{2}\KL\pa{\P_{0}^{\hist_H^T}, \P_{(h^*,a^*)}^{\hist_H^T}}}.
	\end{align*}
	Lemma~\ref{lemma:kl-between-mdps} yields
	\begin{align*}
	\KL\pa{\P_{0}^{\hist_H^T}, \P_{(h^*,a^*)}^{\hist_H^T}} = \EEs{0}{N_{(h^*,a^*)}}\kl(1/2, 1/2+\epsilon)
	\end{align*}
	since $\mdp_0$ and $\mdp_{(h^*,a^*)}$ only differ at stage $h^*$ when $(s, a) = (s_1, a^*)$.

	Assuming that $\epsilon \leq 1/4$, we have $\kl(1/2, 1/2+\epsilon) \leq 4\epsilon^2$ by Lemma \ref{lemma:kl-epsilon}, and, consequently


	\begin{align*}
	\frac{1}{T}\EEs{(h^*,a^*)}{N_{(h^*,a^*)}} \leq \frac{1}{T}\EEs{0}{N_{(h^*,a^*)}} +  \sqrt{2}\epsilon \sqrt{\EEs{0}{N_{(h^*,a^*)}}}.
	\end{align*}
	Averaging over $(h^*,a^*)\in\braces{2, \overline{H}+1}\times\cA$ and using the fact that $\sum_{(h^*,a^*)}N_{(h^*,a^*)} = T$, we obtain
	\begin{align}
	\frac{1}{\overline{H}AT}\sum_{(h^*,a^*)}\EEs{(h^*,a^*)}{N_{(h^*,a^*)}} & \leq \frac{1}{\overline{H}A} + \frac{\sqrt{2}\epsilon}{\overline{H}A} \sum_{(h^*,a^*)}\sqrt{\EEs{0}{N_{(h^*,a^*)}}} \nonumber\\
	& \leq \frac{1}{\overline{H}A} + \frac{\sqrt{2}\epsilon}{\overline{H}A}\sqrt{\overline{H}AT}
	\quad\text{by the Cauchy-Schwarz inequality.} \label{eq:aux4}
	\end{align}

	\paragraph{Optimizing $\epsilon$ and choosing $\overline{H}$} Let $\overline{H} = H/2$ and assume $H \geq 4$. Putting together equations \eqref{eq:aux3} and \eqref{eq:aux4}, we obtain
	\begin{align*}
	\max_{(h^*,a^*)} \regret_T(\histpi, \mdp_{(h^*,a^*)})
	& \geq T\pa{\frac{H}{2}-1}\epsilon\pa{1-\frac{2}{HAT}\sum_{(h^*,a^*)}\EEs{(h^*,a^*)}{N_{(h^*,a^*)}}}
	\\
	&
	\geq \frac{TH}{4}\epsilon\pa{1-\frac{2}{HA}-\frac{2\epsilon}{HA}\sqrt{HAT}}.
	\end{align*}
	Taking $\epsilon = \frac{1}{4}\pa{ 1-\frac{2}{HA}}\sqrt{\frac{HA}{T}}$ yields
	\begin{align*}
	\max_{(h^*,a^*)} \regret_T(\histpi, \mdp_{(h^*,a^*)})
	\geq \frac{1}{32}\pa{1-\frac{2}{HA}}^2 H \sqrt{HAT} \geq \frac{1}{128} H \sqrt{HAT}.
	\end{align*}
	Finally, notice that the assumption $\epsilon\leq 1/4$ is satisfied if $T\geq HA$.
\end{proof}

